eMEM: A Hybrid Spatio-Temporal Memory System For Embodied Agents

We present eMEM (Embodied Memory), a hybrid graph-based memory system for embodied agents operating in physical environments. Current agent memory architectures, such as Generative Agents, MemGPT, and A-MEM, treat memory as text streams or knowledge graphs, but embodied agents require memory that is simultaneously searchable by meaning, space, and time. eMEM fills this gap with a multi-index architecture (SQLITE for structured storage, hnswlib for approximate nearest neighbour semantic search, and an R-tree for spatial queries) unified behind a single graph model. A tiered consolidation pipeline transforms raw perceptual observations into compressed summaries, mirroring hippocampal-neocortical consolidation in biological systems. Ten agent-facing recall tools expose memory retrieval primitives, including concept-to-location resolution and cross layer recall, as first-class operations for LLM tool calling. The system is fully embedded and runs in-process alongside the agent. In addition we introduce eMEM-Bench v1, a benchmark we construct over ProcTHOR-10K scenes for embodied memory evaluation. The benchmark is organised explicitly around eight cognitive-psychology paradigms (DRM lures, pattern separation, pattern completion, source monitoring, context-dependent retrieval, long-horizon interference, serial position, and a foil augmented retention curve), each chosen so that the result is interpretable against the broader memory-systems literature in humans and prior agent-memory systems; a level of diagnostic that surface-task benchmarks like LoCoMo or OpenEQA cannot provide. eMEM scores 80.8 weighted mean over 988 probes, with a flat retention curve at ceiling from 1 h to 1 yr of simulated delay on room-unique items. We show that a pure RAG baseline (the flat_rag ablation) loses 30 pt on context dependent retrieval and 29 pt on DRM lure rejection, isolating the contribution of multi-layer storage and consolidation respectively. We release both the system and the benchmark code.

==> figures/storage_indices.tex <==
% TikZ: SQLite + HNSW + R-tree. Figure 4 (P1).
\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \node[draw, rounded corners] (placeholder) {Storage indices placeholder};
  \end{tikzpicture}
  \caption{Three-index storage: SQLite, HNSW, R-tree.}
  \label{fig:storage-indices}
\end{figure}


==> tables/flat_rag_ablation.tex <==
% flat_rag ablation results vs full baseline.
\begin{table}[t]
  \centering
  \small
  \begin{tabular}{l r r r r}
    \toprule
    \textbf{Paradigm} & $n$ & \textbf{flat\_rag} & \textbf{full (headline)} & $\Delta$ \\
    \midrule
    serial\_position             & 13  & 69.2 & 69.4 &  $0.0$  \\
    retention\_interval\_decay   & 36  & 86.1 & 89.1 & $-3.0$  \\
    pattern\_separation          & 53  & 60.9 & 71.7 & $-10.8$ \\
    long\_horizon\_interference  & 54  & 57.4 & 69.4 & $-11.9$ \\
    pattern\_completion          & 30  & 66.7 & 79.5 & $-12.8$ \\
    source\_monitoring           & 22  & 61.4 & 78.6 & $-17.2$ \\
    DRM                          & 19  & 57.9 & 86.7 & $-28.8$ \\
    context\_dependent\_retrieval&  6  & 33.3 & 63.8 & $-30.5$ \\
    \midrule
    \textbf{Weighted overall}    & \textbf{233} & \textbf{${\sim}64.3$} & \textbf{80.8} & \textbf{$-16.5$} \\
    \bottomrule
  \end{tabular}
  \caption{\texttt{flat\_rag} (pure RAG: no consolidation, no
  multi-layer storage, only \texttt{semantic\_search} and
  \texttt{temporal\_query}) vs.\ \texttt{full} on eMEM-Bench v1
  paradigms. $n$ is the number of probes for the flat\_rag cell
  ($n=6$ schedule cap per cell, but per-paradigm probe yields vary
  with batching). The \texttt{full (headline)} column reproduces the
  un-capped numbers from Table~\ref{tab:emem-bench-v1}; the
  n-matched \texttt{full} baseline run is in progress. The gap
  concentrates on paradigms whose answers require structure
  (DRM, source monitoring, context-dependent retrieval) and
  disappears on paradigms whose answers are vector-search friendly
  (serial position, yes/no retention).}
  \label{tab:flat-rag-ablation}
\end{table}


==> tables/retention_curve.tex <==
% Retention curve from the retention_interval_decay paradigm.
\begin{table}[t]
  \centering
  \small
  \begin{tabular}{l r r r r}
    \toprule
    \textbf{Delay} & \textbf{Hit rate} & \textbf{Correct-reject} & \textbf{False-alarm} & $N$ \\
    \midrule
    1\,h    & 100.0\% & 76.3\% & 15.8\% & 77 \\
    1\,d    & 100.0\% & 79.5\% & 15.4\% & 78 \\
    1\,wk   & 100.0\% & 79.5\% & 15.4\% & 78 \\
    1\,mo   & 100.0\% & 79.5\% & 15.4\% & 78 \\
    6\,mo   & 100.0\% & 79.5\% & 15.4\% & 78 \\
    1\,yr   & 100.0\% & 79.5\% & 15.4\% & 78 \\
    \bottomrule
  \end{tabular}
  \caption{eMEM retention over six delay buckets. Hit rate is $P(\text{yes}\mid\text{seen})$
  on probes asking ``Did you see the $X$?'' where $X$ was perceived
  during the trajectory. Correct-reject is the analogue for foil
  probes where $X$ was absent from the scene. Verdicts are derived
  from log parsing; per-delay totals differ slightly because ambiguous
  predictions are reported separately. The curve is \emph{flat at
  ceiling} on seen items from 1\,h to 1\,yr of simulated delay: no
  measurable forgetting on room-unique items across the full range.
  The ${\sim}\,15.5$\% false-alarm rate is constant across delays and
  is item-level (six foils are consistently confusable), not
  time-dependent.}
  \label{tab:retention-curve}
\end{table}

